MSR-GAN: Multi-Segment Reconstruction via Adversarial Learning

Multi-segment reconstruction (MSR) is the problem of estimating a signal given noisy partial observations. Here each observation corresponds to a randomly located segment of the signal. While previous works address this problem using template or moment-matching, in this paper we address MSR from an unsupervised adversarial learning standpoint, named MSR-GAN. We formulate MSR as a distribution matching problem where the goal is to recover the signal and the probability distribution of the segments such that the distribution of the generated measurements following a known forward model is close to the real observations. This is achieved once a min-max optimization involving a generator-discriminator pair is solved. MSR-GAN is mainly inspired by CryoGAN [1]. However, in MSR-GAN we no longer assume the probability distribution of the latent variables, i.e. segment locations, is given and seek to recover it alongside the unknown signal. For this purpose, we show that the loss at the generator side originally is non-differentiable with respect to the segment distribution. Thus, we propose to approximate it using Gumbel-Softmax reparametrization trick. Our proposed solution is generalizable to a wide range of inverse problems. Our simulation results and comparison with various baselines verify the potential of our approach in different settings.

==> figs/viz_signals.tex <==
% the pdf plots
\begin{figure*}[h]%\centering
\centering
	\begin{tikzpicture}
		\begin{groupplot}[group style={group size= 4 by 3,                      % taille du group plot
    				horizontal sep=0.6cm, vertical sep=1.cm},     
	            	 legend pos= south west,        % Position de la légende dans les figures
					 legend style={at={(0.45,0.5)}, legend cell align=left, draw=none, fill=none},
					 grid=both,                         % grid
    				 height=3.5cm,width=5.4cm,
    				 xmin=1,xmax=64,
					 ymin=-0.1,ymax=1, 
					 ylabel near ticks, xlabel near ticks, xlabel style={align=center,text width=3cm},
					 yticklabel style = {font=\tiny,yshift=0.5ex},
					 xticklabel style = {font=\tiny,xshift=0.5ex},] 
		% sinosoid signal
		\nextgroupplot[title={Known PMF},xticklabels={,,},xlabel={\textcolor{darkblue}{$\textrm{Rel-Error}=0.0002$} \textcolor{darkred}{$\textrm{Rel-Error}=0.0026$}},ymin=-1,ymax=1, x label style={at={(axis description cs:0.5,0)},anchor=north}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_est_known_sin.dat};
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/1_est_known_sin.dat};
			 \addplot[darkgreen,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_gt_known_sin.dat};
		\legend{{\tiny $\textrm{SNR}=\infty$ },{\tiny $\textrm{SNR}=1$ } ,{\tiny GT}};
		\nextgroupplot[title={Fixed PMF with Unif.}, xticklabels={,,},xlabel={\textcolor{darkblue}{$\textrm{Rel-Error}=0.8346$} \textcolor{darkred}{$\textrm{Rel-Error}=2.5409$}},ymin=-2,ymax=2, x label style={at={(axis description cs:0.5,0)},anchor=north}] 	
			\addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_est_fixed_sin.dat};
			\addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/1_est_fixed_sin.dat};
			\addplot[darkgreen,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_gt_fixed_sin.dat};
		\nextgroupplot[title={Unknown PMF}, xticklabels={,,},xlabel={\textcolor{darkblue}{$\textrm{Rel-Error}=0.0119$} \textcolor{darkred}{$\textrm{Rel-Error}=0.1097$}},ymin=-1.2,ymax=1.2, x label style={at={(axis description cs:0.5,0)},anchor=north}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_est_unknown_sin.dat};	
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/1_est_unknown_sin.dat};	
			 \addplot[darkgreen,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_gt_unknown_sin.dat};
	    \nextgroupplot[title={MSR-GAN est. PMF vs GT},xticklabels={,,},xlabel={\textcolor{darkblue}{$\textrm{TV}=0.058$} \textcolor{darkred}{$\textrm{TV}=0.079$}}, ymin=0,ymax=0.04, x label style={at={(axis description cs:0.5,0)},anchor=north}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_est_pdf_sin.dat};	
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/1_est_pdf_sin.dat};	
			 \addplot[darkgreen,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_gt_pdf_sin.dat};
			 %\legend{{\footnotesize Est. PMF },{\footnotesize GT }}
		% tri signal
		\nextgroupplot[xticklabels={,,},xticklabels={,,},xlabel={\textcolor{darkblue}{$\textrm{Rel-Error}=0.0151$} \textcolor{darkred}{$\textrm{Rel-Error}=0.0367$}},ymin=-0.1,ymax=1, x label style={at={(axis description cs:0.5,0)},anchor=north}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_est_known_tri.dat};
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/1_est_known_tri.dat};
			 \addplot[darkgreen,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_gt_known_tri.dat};
		\nextgroupplot[xticklabels={,,},xticklabels={,,},xlabel={\textcolor{darkblue}{$\textrm{Rel-Error}=2.38$} \textcolor{darkred}{$\textrm{Rel-Error}=1.45$}},ymin=-2,ymax=3, x label style={at={(axis description cs:0.5,0)},anchor=north}] 	
			\addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_est_fixed_tri.dat};
			\addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/1_est_fixed_tri.dat};
			\addplot[darkgreen,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_gt_fixed_tri.dat};
		\nextgroupplot[xticklabels={,,},xlabel={\textcolor{darkblue}{$\textrm{Rel-Error}=0.0082$} \textcolor{darkred}{$\textrm{Rel-Error}=0.0888$}}, x label style={at={(axis description cs:0.5,0)},anchor=north}, ymin=-0.1,ymax=1.2] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_est_unknown_tri.dat};
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/1_est_unknown_tri.dat};
			 \addplot[darkgreen,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_gt_unknown_tri.dat};
	    \nextgroupplot[xticklabels={,,},xlabel={\textcolor{darkblue}{$\textrm{TV}=0.070$} \textcolor{darkred}{$\textrm{TV}=0.074$}},ymin=0,ymax=0.03, x label style={at={(axis description cs:0.5,0)},anchor=north}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_est_pdf_tri.dat};	
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/1_est_pdf_tri.dat};	
			 \addplot[darkgreen,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_gt_pdf_tri.dat};
		% random signal
		\nextgroupplot[xticklabels={,,},xticklabels={,,},xlabel={\textcolor{darkblue}{$\textrm{Rel-Error}=0.0036$} \textcolor{darkred}{$\textrm{Rel-Error}=0.1764$}},ymin=-0.5,ymax=0.8, x label style={at={(axis description cs:0.5,0)},anchor=north}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_est_known_rand.dat};
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/1_est_known_rand.dat};
			 \addplot[darkgreen,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_gt_known_rand.dat};
		\nextgroupplot[xticklabels={,,},xticklabels={,,},xlabel={\textcolor{darkblue}{$\textrm{Rel-Error}=0.42$} \textcolor{darkred}{$\textrm{Rel-Error}=0.44$}},ymin=-0.7,ymax=0.8, x label style={at={(axis description cs:0.5,0)},anchor=north}] 	
			\addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_est_fixed_rand.dat};
			\addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/1_est_fixed_rand.dat};
			\addplot[darkgreen,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_gt_fixed_rand.dat};
		\nextgroupplot[xticklabels={,,},xlabel={\textcolor{darkblue}{$\textrm{Rel-Error}=0.01$} \textcolor{darkred}{$\textrm{Rel-Error}=0.11$}},ymin=-0.7,ymax=0.7, x label style={at={(axis description cs:0.5,0)},anchor=north}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_est_unknown_rand.dat};
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/1_est_unknown_rand.dat};
			 \addplot[darkgreen,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_gt_unknown_rand.dat};
	    \nextgroupplot[xticklabels={,,},xlabel={\textcolor{darkblue}{$\textrm{TV}=0.065$} \textcolor{darkred}{$\textrm{TV}=0.135$}}, ymin=0,ymax=0.05, x label style={at={(axis description cs:0.5,0)},anchor=north}] 	
			 \addplot[darkblue,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_est_pdf_rand.dat};
			 \addplot[darkred,very thick] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/1_est_pdf_rand.dat};
			 \addplot[darkgreen,very thick,dashdotted] table[x=x, y=y, col sep=comma]{figs/viz_signals_dat/0_gt_pdf_rand.dat};
			 %\legend{{\footnotesize Initial $\theta_3$ },{\footnotesize Ours $\theta_3$ },{\footnotesize Relion $\theta_3$ }};
		\end{groupplot}
	\end{tikzpicture}
\caption{Comparison between MSR-GAN in different noise regimes for 1) known PMF (first column), 2) unknown PMF but fixed with uniform distribution during training (second column), 3) unkown PMF and recovered during training (third column). The last column plots the ground truth PMF (green dashed curve) alongside the estimated PMFs from MSR-GAN (the same experiment as the third column) in blue and red. Each row corresponds to different signals and PMFs. The relative error of the reconstruction for $\textrm{SNR}=\infty$ and $\textrm{SNR}=1$ is written in blue ($\textrm{SNR}=\infty$) and red ($\textrm{SNR}=1$) underneath each subplot. For all experiments in this figure we are using the same architecture for the discriminator with $\ell=100$ and the number of measurements is $N=5 \times 10^4$.}
\label{fig:signal_viz_results}
\end{figure*}
